Oscillations enhance time-series prediction in reservoir computing with feedback

Reservoir computing, a machine learning framework used for modeling the brain, can predict temporal data with little observations and minimal computational resources. However, it is difficult to accurately reproduce the long-term target time series because the reservoir system becomes unstable. This predictive capability is required for a wide variety of time-series processing, including predictions of motor timing and chaotic dynamical systems. This study proposes oscillation-driven reservoir computing (ODRC) with feedback, where oscillatory signals are fed into a reservoir network to stabilize the network activity and induce complex reservoir dynamics. The ODRC can reproduce long-term target time series more accurately than conventional reservoir computing methods in a motor timing and chaotic time-series prediction tasks. Furthermore, it generates a time series similar to the target in the unexperienced period, that is, it can learn the abstract generative rules from limited observations. Given these significant improvements made by the simple and computationally inexpensive implementation, the ODRC would serve as a practical model of various time series data. Moreover, we will discuss biological implications of the ODRC, considering it as a model of neural oscillations and their cerebellar processors.

==> Makefile <==
######################
# Makefile for Latex #
######################
      SRC_NAME = nn
INPUT_SRC_NAME = 
           SRC = $(SRC_NAME).tex
     INPUT_SRC = $(SUB_SRC_NAME).tex
      AUX_FILE = ${SRC_NAME}.aux
      BBL_FILE = ${SRC_NAME}.bbl
      BLG_FILE = ${SRC_NAME}.blg
      DVI_FILE = ${SRC_NAME}.dvi
      PDF_FILE = ${SRC_NAME}.pdf
      LOF_FILE = ${SRC_NAME}.lof
      LOG_FILE = ${SRC_NAME}.log
      LOT_FILE = ${SRC_NAME}.lot
      TOC_FILE = ${SRC_NAME}.toc
      ENT_FILE = ${SRC_NAME}.ent
      FFF_FILE = ${SRC_NAME}.fff
      TTT_FILE = ${SRC_NAME}.ttt
       RM_FILE = ${AUX_FILE} ${BBL_FILE} ${BLG_FILE} \
                 ${LOF_FILE} ${LOG_FILE} ${LOT_FILE} \
                 ${TOC_FILE} ${ENT_FILE} ${FFF_FILE} \
		 ${TTT_FILE} core* *~		

         LATEX = latex
	BIBTEX = bibtex
          XDVI = xdvi
	  PDFM = dvipdfmx
	  ACRO = open -a "preview"
            RM = /bin/rm -f

.SUFFIXRS : .tex

all :
	$(LATEX) $(SRC_NAME)
	$(BIBTEX) $(SRC_NAME)
	$(LATEX) $(SRC_NAME)
	$(LATEX) $(SRC_NAME)
	$(PDFM) $(DVI_FILE)
	$(ACRO) $(PDF_FILE) &

one :
	$(LATEX) $(SRC_NAME)

x :
	$(XDVI) $(DVI_FILE) &

a :
	$(PDFM) $(DVI_FILE)
	$(ACRO) $(PDF_FILE) &

clean:
	@ $(RM) $(RM_FILE)



